ExplainIt! -- A declarative root-cause analysis engine for time series data (extended version)

We present ExplainIt!, a declarative, unsupervised root-cause analysis engine that uses time series monitoring data from large complex systems such as data centres. ExplainIt! empowers operators to succinctly specify a large number of causal hypotheses to search for causes of interesting events. ExplainIt! then ranks these hypotheses, reducing the number of causal dependencies from hundreds of thousands to a handful for human understanding. We show how a declarative language, such as SQL, can be effective in declaratively enumerating hypotheses that probe the structure of an unknown probabilistic graphical causal model of the underlying system. Our thesis is that databases are in a unique position to enable users to rapidly explore the possible causal mechanisms in data collected from diverse sources. We empirically demonstrate how ExplainIt! had helped us resolve over 30 performance issues in a commercial product since late 2014, of which we discuss a few cases in detail.

==> Makefile <==
# http://vldb.org/2019/?formatting-guidelines
TARGET=explainit
BIBTEX := bibtex
OS := $(shell uname)
SOURCES=$(TARGET).tex $(wildcard *.tex) $(wildcard images/*)\
    $(TARGET).bib

all: $(TARGET).pdf

ifeq ($(OS), Darwin)
$(TARGET).pdf: $(SOURCES)
#	pdflatex $(TARGET).tex
#	$(BIBTEX) $(TARGET)
#	pdflatex $(TARGET)
#	pdflatex $(TARGET)
#	grep undef *.log || true
	latexmk -pdf $(TARGET).tex
else
$(TARGET).pdf: $(SOURCES)
	latexmk -pdf -interaction=nonstopmode -halt-on-error \
			-file-line-error $(TARGET).tex
endif

pdf: $(TARGET).pdf
	xpdf $(TARGET).pdf

view: $(TARGET).pdf
	open $(TARGET).pdf

clean:
	latexmk -quiet -C $(TARGET).tex
	rm -f `cat .gitignore` .*~
	@extraneous=`git ls-files -o`; if test -n "$$extraneous"; then \
		echo WARNING:  The following files are not in git:; \
		printf "        %s\n" $$extraneous; \
		exit 1; \
	fi
#	rm -f *.aux *.log *.out *.bbl *.blg *~ *.bak *.synctex.gz $(TARGET).pdf


==> architecture.tex <==
% ingest


==> jdb <==
JMLR:::: Journal of Machine Learning Research;;;;JMLR
COLT:::: Proceedings of the 26th Annual Conference on Learning Theory (COLT 2013)
http://spark.apache.org:::: URL http://spark. apache. org;;;;http://spark.apache.org
Causal ML Workshop at ICML 2018:::: Causal ML Workshop at ICML 2018
The Journal of experimental education:::: The Journal of experimental education
Wiley:::: JOHN WILEY \& SONS, INC., 605 THIRD AVE., NEW YORK, NY 10158, USA, 1983, 512
ICDM:::: Data Mining, 2008. ICDM'08. Eighth IEEE International Conference on;;;;Data Mining (ICDM), 2014 IEEE International Conference on;;;;ICDM
Statistica Neerlandica:::: Statistica Neerlandica
The Stanford Encyclopedia of Philosophy:::: The Stanford Encyclopedia of Philosophy
SIGMOD:::: Proceedings of the 2014 ACM SIGMOD international conference on Management of data;;;;Proceedings of the 2017 ACM International Conference on Management of Data;;;;SIGMOD
SIGKDD:::: Proceedings of the ninth ACM SIGKDD international conference on Knowledge discovery and data mining;;;;Proceedings of the 23rd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining;;;;Proceedings of the 21th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining;;;;Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining;;;;SIGKDD
Science:::: Science
Statistics surveys:::: Statistics surveys
OSDI:::: OSDI
VLDB:::: Proceedings of the VLDB Endowment;;;;VLDB
CACM:::: Communications of the ACM
CausalML Workshop, ICML:::: CausalML Workshop, ICML
TOIS:::: ACM Transactions on Information Systems (TOIS)
Journal of econometrics:::: Journal of econometrics
Journal of the royal statistical society. Series B (Methodological):::: Journal of the royal statistical society. Series B (Methodological)
Journal of Neuroscience:::: Journal of Neuroscience
NIPS:::: NIPS


==> schema.tex <==
\sys expects the input t

